ROSCOE: A Suite of Metrics for Scoring Step-by-Step Reasoning

Large language models show improved downstream task performance when prompted to generate step-by-step reasoning to justify their final answers. These reasoning steps greatly improve model interpretability and verification, but objectively studying their correctness (independent of the final answer) is difficult without reliable methods for automatic evaluation. We simply do not know how often the stated reasoning steps actually support the final end task predictions. In this work, we present ROSCOE, a suite of interpretable, unsupervised automatic scores that improve and extend previous text generation evaluation metrics. To evaluate ROSCOE against baseline metrics, we design a typology of reasoning errors and collect synthetic and human evaluation scores on commonly used reasoning datasets. In contrast with existing metrics, ROSCOE can measure semantic consistency, logicality, informativeness, fluency, and factuality - among other traits - by leveraging properties of step-by-step rationales. We empirically verify the strength of our metrics on five human annotated and six programmatically perturbed diagnostics datasets - covering a diverse set of tasks that require reasoning skills and show that ROSCOE can consistently outperform baseline metrics.

==> tables/table-corr-syn-sup-SIMPLE.tex <==
\begin{table*}[!b]
  \centering
  \footnotesize
  \setlength\tabcolsep{3.4pt}
    \vspace{-8pt}
  \renewcommand{\arraystretch}{1}
        \caption{\footnotesize Kendall's $\tau$ correlation of different metrics on six \textbf{Diagnostics} datasets. Metrics are measured \textbf{reference-based} on $(\bm{s},\bm{h})$. We take the maximum over different perturbations (see $\S$\ref{diagnostics-experiments}). 
        % We report the highest correlation scores across perturbations within each dataset. 
        The highest and second best correlation for each dataset are in \textbf{bold} and underlined, respectively. Breakdown of all baseline and \ourmodel~ metrics are shown in App.~\ref{app:diagnostics-experiments}, Table~\ref{tab:corr-synth-sup-max}. 
        }
    \scalebox{0.86}
    {
        \begin{tabular}{@{}l@{}c@{}c@{}c@{}c@{}c@{}c@{}}
    \toprule
          & \textbf{\hyperref[tab:corr-synth-unsup-perturb-entbank]{\underline{EntBank}}} \ \ &
          \textbf{\hyperref[tab:corr-synth-unsup-perturb-math]{\underline{Math}}} \ \ & 
          \textbf{\hyperref[tab:corr-synth-unsup-perturb-aqua]{\underline{AQUA}}} \ \ & 
          \textbf{\hyperref[tab:corr-synth-unsup-perturb-proofwriter]{\underline{ProofWr.}}} \ \ & 
          \textbf{\hyperref[tab:corr-synth-unsup-perturb-eqasc]{\underline{EQASC}}} \ \ & 
          \textbf{\hyperref[tab:corr-synth-unsup-perturb-asdiv]{\underline{ASDIV}}} \\ 
   ROUGE-L & \textbf{0.818}	& \underline{0.812}	 &	\textbf{0.819} & \textbf{0.821}	& \textbf{0.822}	& \textbf{0.899} \\ 
   BLEURT & 0.556	& 0.544	&0.544	& 0.497	& 0.708	& 0.659 \\
   BERTScore	& 0.748	& 0.708	&0.747	& 0.738	& 0.736	& 0.736 \\ 
   \bartscore & 0.707	& 0.686	&0.708	& 0.703	& 0.708	& 0.722 \\
   \bartscoreParaCnn & 0.682	& 0.674 &	0.681	& 0.688	& 0.700	& 0.711 \\
   \bartscoreFineTuned & 0.686	& 0.593	&	0.677& 0.526	& 0.563	& 0.614 \\
   PRISM & 0.648	& 0.354	&	0.677& 0.702	& 0.705	& 0.722 \\
   CTC Relev. & 0.440	& 0.553	&	0.602& 0.469	& 0.706	& 0.428 \\
   CTC Consist. & 0.272	& 0.193 &		0.131	& 0.358	& 0.174	& 0.334 \\
\midrule
\ourmodelsa	& \underline{0.814}	& \textbf{0.817}	& 0.819	& \underline{0.814}	& \underline{0.805}	& \underline{0.817} \\
\ourmodelsa^1	& 0.779	& 0.648	& \textbf{0.819}	& 0.782	& 0.775	& \underline{0.817} \\
\ourmodelsa^2	& 0.814	& 0.817	& \textbf{0.819}	& 0.814	& 0.802	& \underline{0.817} \\
\midrule
\ourmodelss	& 0.763	& 0.762	& 0.771	& 0.769	& 0.763	& 0.771 \\
\ourmodelss^1	& 0.766	& 0.749	& 0.774	& 0.765	& 0.757	& 0.765 \\
\ourmodelss^2	& 0.761	& 0.761	& 0.764	& 0.766	& 0.760	& 0.782 \\
    \bottomrule
    \end{tabular}
    }
      \vspace{-10pt}
  \label{tab:corr-synth-sup-simple}%
\end{table*}%

% BARTScore_Recall	0.708
% BARTScore_Faithful1lness	0.708
% BARTScore_Informativeness	0.707
% BERTScore_P	0.747
% BERTScore_R	0.749
% BERTScore_F	0.747
% Rouge_1	0.819
% Rouge_2	0.819
% Rouge_L	0.819
% CTC_relevance	0.602
% CTC_consistency	0.131
% bart_score_para_hypo_ref	0.690
% bart_score_para_ref_hypo	0.650
% bart_score_paraavg_f	0.681
% bart_score_para_harm_f	0.686
% prism_ref_hypo	0.666
% prism_hypo_ref	0.675
% prism_avg	0.677
% BLEURT	0.544
% Finetuned-BARTScore_Recall	0.655
% Finetuned-BARTScore_Faithful1lness	0.677
% Finetuned-BARTScore_Informativeness	0.667
% \begin{table*}[!t]


==> tables/table-human-evalution-perspectives.tex <==

\begin{wraptable}{r}{6.8cm}
\centering
% \renewcommand{\arraystretch}{0.95}
% \setlength\tabcolsep{4.4pt}
  \footnotesize
  \vspace{-10pt}
        \caption{\label{tab:humanperspectives} \footnotesize Reasoning evaluation perspectives in human judged datasets (see details in Table~\ref{tab:human-eval-perspectives}). \asli{@Olga/Spencer, need to revise this table.}
        }    
    \scalebox{0.9}
	    {
    \begin{tabular}{@{}l|l@{}}
    \toprule
    \textbf{Overall Sequence (\texttt{SEQ})} & \textbf{Step-Level (\texttt{STEP})}\\
    \midrule     
    \texttt{QUAL}: Quality &  \texttt{S-FACT}: Factuality \\
    \texttt{COH}: Coherence  & \texttt{S-RED}:  Redundancy\\
    \texttt{CON-SO}: Source-Consistency  & \texttt{S-HALL}:  Hallucination\\
    \texttt{CON-SE}: Self-Consistency & \texttt{S-COV}: Coverage\\
   \texttt{MISS}: Missing Step  &  \texttt{S-LOG}: Logical Error \\
\bottomrule
    % \vspace{-15pt}
 \end{tabular}%
 }
     \vspace{5pt}
%\end{wraptable}
\end{wraptable}


% \begin{wrapfigure}{r}{0.5\textwidth}
%   \vspace{-20pt}
%   \begin{center}
%     \includegraphics[width=0.48\textwidth]{gull}
%   \end{center}
%   \vspace{-20pt}
%   \caption{A gull}
%   \vspace{-10pt}
% \end{wrapfigure}

==> tables/table-intofigure.tex <==

\begin{table}[t]
\caption{Step-by-step reasoning generated from 2-shot PALM \citep{wei2022chain} and GPT-3 (text-davinci-002) \citep{brown2020language}. Different error types are highlighted: \hlc[pink]{logical or factual issues}, \hlc[yellow]{irrelevant to the question}, \hlc[mygreen]{somewhat-relevant}. Full 2-shot exemplars are shown in Appendix~\ref{app:intro}.}
\small
\vspace{-10}
\fbox{
\scalebox{0.83}
	    {
\begin{minipage}{.58\textwidth}
\begin{singlespace}
\textbf{\ul{Example #1}} \\
\textbf{Context}: Jennifer looked out her window and saw a really cool cloud below her. She unbuckles her seatbelt and heads to the bathroom. \\
\textbf{Question}: Is Jennifer probably traveling more than 300 miles per hour relative to the earth? \\

\textbf{PALM Step-by-step reasoning (Correct)}

\noindent $\ \ \ \bullet$ {300 miles per hour is about 480 km/h.}


\noindent $\ \ \ \bullet$ {This is about the speed of a commercial airplane.}

\noindent $\ \ \ \bullet$ {Clouds are usually below airplanes, so Jennifer is probably on an airplane.} 

\noindent $\ \ \ \bullet$ {The answer is yes.} \\

\textbf{GPT-3 Step-by-step reasoning (Incorrect)}

\noindent $\ \ \ \bullet$ \hlc[pink]{No, because an airplane typically travels around 500-600 miles per hour.}

\noindent $\ \ \ \bullet$ \hlc[yellow]{The bathroom is usually located in the back of the plane.}
\end{singlespace}%
\end{minipage}
}}\kern3pt%
\fbox{
\scalebox{0.83}
	    {
\begin{minipage}{.55\textwidth}
\begin{singlespace*}
\textbf{\ul{Example #2}} \\
\textbf{Context}: Shelley is from Virginia, but is visiting that city with that famous market where they throw the fish. Going home next Tuesday! \\
\textbf{Question}: Is it likely that Shelly will be near the Pacific Ocean this weekend?\\

\textbf{GPT-3 Step-by-step reasoning (Partially correct)}


\noindent $\ \ \ \bullet$ \hlc[pink]{No, it is not likely that Shelley will be near the Pacific Ocean this weekend.} 

\noindent $\ \ \ \bullet$ \hlc[mygreen]{Shelley is from Virginia, which is on the East Coast of the United States.} 
% \hlc[orange]{Shelley is from Virginia, which is on the East Coast of the United States.} 

\noindent $\ \ \ \bullet$ {The Pacific Ocean is on the West Coast.} 

\noindent $\ \ \ \bullet$ \hlc[yellow]{Shelley is visiting a city with a famous market, which could be anywhere in the world.}

\noindent $\ \ \ \bullet$ \hlc[pink]{Tuesday is her travel day, so she will likely not be traveling this weekend.}
\end{singlespace*}
\end{minipage}
}}
\label{introfigure}
\end{table}
